Composing Copyless Streaming String Transducers

Streaming string transducers (SSTs) implement string-to-string transformations by reading each input word in a single left-to-right pass while maintaining fragments of potential outputs in a finite set of string variables. These variables get updated on transitions of the transducer, where they can be assigned new values described by concatenations of variables and output symbols. An SST is called copyless if every update is such that no variable occurs more than once amongst all of the assigned expressions. The transformations realized by copyless SSTs coincide with Courcelle's monadic second-order logic graph transducers (MSOTs) when restricted to string graphs. Copyless SSTs with nondeterminism are known to be equivalent to nondeterministic MSOTs as well. MSOTs, both deterministic and nondeterministic, are closed under composition. Given the equivalence of MSOTs and copyless SSTs, it is easy to see that copyless SSTs are also closed under composition. The original proof of this fact, however, was based on a direct construction to produce a composite copyless SST from two given copyless SSTs. A counterexample discovered by Joost Englefriet showed that this construction may produce copyful transducers. We revisit the original composition constructions for both deterministic and nondeterministic SSTs and show that, although they can introduce copyful updates, the resulting copyful behavior they exhibit is superficial. To characterize this mild copyful behavior, we define a subclass of copyful SSTs, called diamond-free SSTs, in which two copies of a common variable are never combined in any subsequent assignment. In order to recover a modified version of the original construction, we provide a method for producing an equivalent copyless SST from any diamond-free copyful SST.

==> nsst.tex <==
Let $T_1 = (\Sigma_1, \Sigma_2, Q, I_1, X, U, \Delta_1, \phi_1)$ and $T_2 = (\Sigma_2, \Sigma_3, P, I_2, Y, A, \Delta_2, \phi_2)$ be copyless \nsst s to be composed.
The composite $T_3 = (\Sigma_1, \Sigma_3, S, I_3, Z, R, \Delta_3, \phi_3)$ will be the result of the following construction.

In the case of \nsst, the composition construction is almost identical to that for \sst.
The main difference is that the maps $f$ and $g$ will be of type $P \times X \to 2^P$ and $P \times X \times Y \to 2^{C(Y, Z, \Sigma_3^*)}$ respectively.
The lifting of these functions to the power sets of their ranges then cascades in the sense that some of the helping functions must be amended to account for this generalization.
The functions $\zeta$ and $\hat{\zeta}$ are however unchanged (cf.~\eqref{eq:zeta} and~\eqref{eq:zetahat}), so we omit their definitions here.
The altered definitions are as follows.

\begin{equation}
\label{eq:fhat_nsst}
\begin{aligned}
	&\hat{f} : (P \times C(X, \Sigma_2^*) \times (P \times X \to P)) \to 2^P \\
	&\hat{f}(p, \mu(x),f) \df \begin{cases}
		\delta_2^*(p,w) & \mu(x) = w \in \Sigma_2^* \\ \\
		f(p, x') & \mu(x) = x' \in X \\ \\
		\bigcup\limits_{p' \in \delta^*_2(p, w)} \hat{f}(p', \mathbf{x}, f) & \mu(x) = w\mathbf{x} \in C(X,\Sigma^*_2) \\ \\
		\bigcup\limits_{p' \in f(p, x')} \hat{f}(p', \mathbf{x}, f) & \mu(x) = x'\mathbf{x} \in C(X,\Sigma^*_2)
	\end{cases}
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:ghat_nsst}
\begin{aligned}
	&\hat{g} : (P \times C(X, \Sigma^*_2) \times C(Y,\Sigma^*_3) \times (P \times X \to P) \times (P \times X \times Y \to C(Y,Z))) \to 2^{C(Y, Z,\Sigma^*_3)} \\
	&\hat{g}(p, \mu(x), \mathbf{y}, f, g) \df \begin{cases}
	\alpha_w(\mathbf{y}) & \begin{aligned}
		&\mu(x) = w \in \Sigma^*_2, \\
		&(p, w, \alpha_w, p') \in \Delta_2^*
		\end{aligned} \\ \\
	g(p, x', \mathbf{y}) & \mu(x) = x' \in X \\ \\
	\bigcup_{p' \in \delta^*_2(p,w)}\bigcup_{\mathbf{y'} \in \alpha_w} \hat{g}(p', \mathbf{x}, \mathbf{y'}, f, g) & \begin{aligned}
		&\mu(x) = w\mathbf{x} \in C(X,\Sigma^*_2), \\
		&(p, w, \alpha_w, p') \in \Delta_2^*
		\end{aligned} \\ \\
	\bigcup_{p' \in f(p,x')}\bigcup_{\mathbf{y'} \in g(p, x', \mathbf{y})} \hat{g}(p', \mathbf{x}, \mathbf{y'}, f, g) & \begin{aligned}
		&\mu(x) = x'\mathbf{x} \in C(X,\Sigma^*_2), \\	
		&(p, \nu(x'), \alpha_{\nu(x')}, p') \in \Delta_2^*
		\end{aligned}
	\end{cases}
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:fancyg_nsst}
\begin{aligned}
	&\mathfrak{g} : (P \times C(X, \Sigma^*_2) \times C(Y,Z,\Sigma_3^*) \times (P \times X \to P) \times (P \times X \times Y \to C(Y,Z))) \to 2^{C(Y,Z,\Sigma^*_3)} \\
	&\mathfrak{g}(p, \mathbf{x}, \mathbf{y}, f, g) \df \bigcup_{(p, \nu(\mathbf{x}), \alpha_{\nu(\mathbf{x})}, p') \in \Delta^*_2} \alpha_{\nu(\mathbf{x})}(\mathbf{y})\big[\forall y \in \mathbf{y}.\ y\big\backslash\hat{g}(p, \mathbf{x}, y, f, g)\big]
\end{aligned}
\end{equation}

Using the above functions, we can construct $T_3$ as follows:
\begin{equation}
\begin{aligned}
	S & \df Q \times [P \times X \to P] \times [P \times X \times Y \to C(Y,Z)]; \\
	I_3 & \df \{(q, (p, x) \mapsto p, (p, x, y_i) \mapsto z_{2i - 1}y_iz_{2i}) : \forall q \in I_1\text{ where }z_{2i-1}, z_{2i} \in Z^x_p\}; \\
	Z & \df \biguplus_{p,x \in P \times X} Z^x_p,\text{ where } |Z^x_p| = 2|Y|, \text{ for all } p \in P \text{ and } x \in X; \\
	\Delta_3 & \df \big\{((q, f, g), \sigma, \varrho, (q', f', g')) : (q, \sigma, \mu, q') \in \Delta_1 \\
	& \qquad \text{ and } f'(p,x) = \hat{f}(p,\mu(x),f) \\
	& \qquad \text{ and } (\varrho, g'(p,x)) \in \bigcup_{\mathbf{v} \in \hat{g}(p,\mu(x), f, g)} \zeta(\mathbf{v}) \big\}; \\
	R & \df \{\varrho : ((q, f, g), \sigma, \varrho, (q', f', g')) \in \Delta_3 \}; \\
	\phi_3((q, f, g)) & \df \bigcup_{\mathbf{x} \in \phi_1(q)} \bigcup_{p_0 \in I_2} \bigcup_{p \in \hat{f}(p_0, \phi_1(q))} \mathfrak{g}(p_0, \mathbf{x}, \phi_2(p), f, g)[\forall y \in Y.\ y\backslash\epsilon] \\
\end{aligned}
\end{equation}

Note that $|S|$ does not change from the deterministic case.
This is because $S$ already is defined to have a state for every possible pair of functions of types $P \times X \to P$ and $P \times X \times Y \to C(Y,Z)$.
Thus, it is not necessary to store more states for the nondeterministic case; it suffices to add in the additional nondeterministic transitions to the same state space.

In Theorem~\ref{theorem:sst_correctness} we showed that a run of the deterministic transducer constructed by the method in Section~\ref{sec:composition} satisfies the correctness invariant.
This was proven by induction on runs through $T_3$, and thereby implies that the invariant holds on any given run.
Thus, any run in $T_3$ that simulates legitimate and corresponding runs in $T_1$ and $T_2$ must satisfy the correctness invariant.
The additional guards placed upon the cases of the helper functions ensure that $T_3$ only simulates these pairs of legitimate runs, and since we've proven runs in $T_3$ to be correct, any individual run in $T_3$ satisfies the deterministic invariant.
Hence, correctness is preserved in the case of \nsst.

\begin{thm}[Correctness for \nsst]
	The following invariant is true at every state in $T_3$:
	If $(q_I, w, \mu_w, q) \in \Delta^*_1$ such that $q_I \in I_1$ and $((q_I,f_0,g_0), w, \varrho_w, (q, f, g)) \in \Delta^*_3$ and $(p, \nu(x), \alpha_{\nu(\mu_w(x))}, p') \in \Delta^*_2$, then $p' \in f(p, x)$ and there exists $\mathbf{z} \in g(p,x,y)$ and $\mathbf{y} \in \alpha_{\nu(\mu_w(x))}(y)$ such that $\nu(\mathbf{z}) = \nu(\mathbf{y})$, for all $y \in Y$.
\end{thm}

==> prelims.tex <==



